Go with the Flow? A Large-Scale Analysis of Health Care Delivery Networks in the United States Using Hodge Theory

Health care delivery is a collaborative process, requiring close coordination among networks of providers with specialized expertise. Yet in the United States, care is often spread across multiple disconnected providers (e.g., primary care physicians, specialists), leading to fragmented care delivery networks, and contributing to higher costs and lower quality. While this problem is well known, there are relatively few quantitative tools available for characterizing care delivery networks at scale, thereby inhibiting deeper understanding of care fragmentation and efforts to address it. In this, study, we conduct a large-scale analysis of care delivery networks across the United States using the discrete Hodge decomposition, an emerging method of topological data analysis. Using this technique, we decompose networks of patient flows among physicians into three orthogonal subspaces: gradient (acyclic flow), harmonic (global cyclic flow), and curl (local cyclic flow). We document substantial variation in the relative importance of each subspace, suggesting that there may be systematic differences in the organization of care delivery networks across health care markets. Moreover, we find that the relative importance of each subspace is predictive of local care cost and quality, with outcomes tending to be better with greater curl flow and worse with greater harmonic flow.

==> tables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% BEGIN REGRESSION TABLE %% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% format page as landscape
%\begin{landscape}

% remove page number
\thispagestyle{empty}
\pagestyle{empty}


{% begin table format

% set font size for table
\scriptsize

% squeeze columns together
\setlength{\tabcolsep}{2pt}

% squeeze rows together
\renewcommand{\arraystretch}{1}

% begin table header
\begin{table}[htbp]\centering

\scalebox{0.8}{%

\begin{threeparttable}
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Regressions predicting cost and quality}
\label{table:RegressionsWeighted}
\begin{tabular}{l*{5}{c}}
\toprule

% add table data
 
                                                                                          &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
                                             &\multicolumn{1}{c}{\shortstack{DV: Total \\ spending per \\ beneficiary \phantom{x} }}&\multicolumn{1}{c}{\shortstack{DV: Inpatient \\ spending per \\ beneficiary \phantom{x} }}&\multicolumn{1}{c}{\shortstack{DV: Outpatient \\ spending per \\ beneficiary \phantom{x} }}&\multicolumn{1}{c}{\shortstack{DV: Readmission \\ rate post-surgical \\ treatment }}&\multicolumn{1}{c}{\shortstack{DV: ER visit \\ rate post-surgical \\ treatment }}\\
\midrule
Gradient flow $g$ per edge                   &         -20.53   &         -33.19   &        -257.18***&          -0.28   &          -0.50   \\
                                             &       (164.71)   &        (99.86)   &        (78.57)   &         (0.86)   &         (0.71)   \\
Harmony flow $h$ per edge                    &        1106.51***&        1114.11***&        2826.45***&           2.26*  &           4.34***\\
                                             &       (323.25)   &       (201.03)   &       (159.67)   &         (1.30)   &         (1.11)   \\
Curl flow $r$ per edge                       &       -1624.75***&       -1364.48***&       -2714.97***&          -2.52***&          -3.52***\\
                                             &       (215.64)   &       (133.91)   &       (104.45)   &         (0.52)   &         (0.51)   \\
Diabetic A1c testing rate                    &         -21.56***&         -16.09***&           5.76***&          -0.06***&          -0.03** \\
                                             &         (5.24)   &         (3.38)   &         (1.74)   &         (0.01)   &         (0.01)   \\
Constant                                     &       12216.94***&        6115.19***&        2052.51***&          16.51***&          19.61***\\
                                             &       (454.57)   &       (294.16)   &       (151.73)   &         (0.88)   &         (1.11)   \\\midrule
Year fixed effects                           &            Yes   &            Yes   &            Yes   &            Yes   &            Yes   \\
\midrule
N                                            &          12925   &          12925   &          12925   &           6034   &           7776   \\
r2                                           &           0.09   &           0.07   &           0.22   &           0.03   &           0.04   \\
 

% add bottom rule
\bottomrule

% close tabular
\end{tabular}

% add table notes
\begin{tablenotes}

\item \emph{Notes:}  The level of analysis is the region $\times$ year. At the edge level, flow values are normalized using the approach described by \cite{schaub2020random}. After summing across edges to define the the region $\times$ year level measures, we divide each sum (i.e., $g$, $h$, $r$) by the total number of edges in the network, as an adjustment for network size. Robust standard errors (clustered on region) are shown in parentheses; p-values correspond to two-tailed tests. 
\item {*}p<0.1; {**}p<0.05; {***}p<0.01

\end{tablenotes}

% close table
\end{threeparttable}
}
\end{table}

% end table format
}%



% end landscape
%\end{landscape}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%% END REGRESSION TABLE %% 
%%%%%%%%%%%%%%%%%%%%%%%%%%

